Restructuring Vector Quantization with the Rotation Trick

Vector Quantized Variational AutoEncoders (VQ-VAEs) are designed to compress a continuous input to a discrete latent space and reconstruct it with minimal distortion. They operate by maintaining a set of vectors -- often referred to as the codebook -- and quantizing each encoder output to the nearest vector in the codebook. However, as vector quantization is non-differentiable, the gradient to the encoder flows around the vector quantization layer rather than through it in a straight-through approximation. This approximation may be undesirable as all information from the vector quantization operation is lost. In this work, we propose a way to propagate gradients through the vector quantization layer of VQ-VAEs. We smoothly transform each encoder output into its corresponding codebook vector via a rotation and rescaling linear transformation that is treated as a constant during backpropagation. As a result, the relative magnitude and angle between encoder output and codebook vector becomes encoded into the gradient as it propagates through the vector quantization layer and back to the encoder. Across 11 different VQ-VAE training paradigms, we find this restructuring improves reconstruction metrics, codebook utilization, and quantization error. Our code is available at https://github.com/cfifty/rotation_trick.

==> sections/challenges.tex <==
\chris{I think this is where we should put all the analysis to motivate what we do. It'll look something like this:}
There appears to be a gap between \textit{trainability} and \textit{expressivity} of VQVAE models. Specifically, VQVAEs are prone to Codebook collapse~\cite{jukebox, videogpt}. We explore the training paradigm and find two explanations: interference between codebook learning and reconstruction and non-accurate gradients through the STE estimator to update the encoder's parameters. 

\textbf{Inferference between codebook learning and Reconstruction}


\textbf{Approximate Encoder Gradients}

==> sections/spherical_code_approximation.tex <==
Spherical codes aim to place $n$ points on a $d$-dimensional hypersphere so that the minimum distance between any two points is maximized. Unfortunately, except for $d=2$, $n + 1 \leq d$, and $d=3$ with $n \in [5, 14] \cup \{24\}$, this has remained an open problem in mathematics for the past 94 years~\citep{tammes}. 

Formally, we consider the $n$ dimensional Euclidean space $\R^d$ equipped with the Euclidean metric $||.||$. For real $r > 0$ and $x \in \R^d$, we define $B_d(x, r)$ to be the open ball of radius $r$ centered at $x$. Let $S^{d - 1}$ be the unit sphere centered at the origin. We define a $\theta$-spherical code as a finite set $A \subset S^{d - 1}$ such that all distinct $x, y \in A$ have an angular separation of at least $\theta$. For a fixed $\theta \in (0, \pi]$, define $M(d, \theta)$ as the cardinality of the $\theta$-spherical code. Notably, $M(d, \theta)$ is equivalent to the largest possible number of unit vectors centered at the origin which have a pairwise angular separation of at least $\theta$.

The spherical codes problem asks, for a fixed $\theta$ and $d$, what is the least upper bound on $M(d, \theta)$. For our problem, we would like to know for a fixed $d$ and $M$, what is the least upper bound on $\rho$. In the Appendix, demonstrate how to use the recent spherical code bounds discovered by \cite{Sardari} to calculate an upper bound on $\rho$. 

In this work, we develop here a collision based algorithm for computing approximate spherical codes. We begin by randomly initializing vectors on $S^{d - 1}$ by sampling from a uniform distribution over the sphere. For each vector $x_m$ in our spherical code, consider the open ball of radius $r$ centered around the head of the vector, $B_m(x_m,r)$. For any other vector $x_k \in A$, we say that the vectors $x_m$ and $x_k$ collide if $B_m(x_m, r) \cap B_k(x_k, r) \neq \emptyset$. We call $r$ the current packing radius. 

Our objective is to maximize the minimum distance $\rho$ for the spherical code. Hence, we would like to maximize the packing radius $r$ while minimizing the volume of the quantity $\bigcup_{k = 1}^M B_k(x_k, r)$ or the overlap between all the balls in the spherical code. We do so as follows. 

We initialize the packing radius as a small value $r_{init}$ which depends on the initial configuration of randomly generated vectors. For a given iteration of the algorithm, we fix a packing radius $r$. A collision occurs between points $x_m$ and $x_k$ in the spherical code if $2 r > d_{m,k}$ where $d_{m,k}$ is the Euclidean distance between $x_m$ and $x_k$. If a collision occurs, we move the two colliding vectors away from each other by a distance proportional to the amount of collision, but if not they remain where they are. That is, for a given pair of vectors $x_m$ and $x_k$, the update vector for $x_m$ is

\[ u_{m,k} = \begin{cases} 
      (x_m - x_k)(2r - d_{m,k}) & : 2r > d_{m,k}\\
      0 & : 2r \leq d_{m,k} \\
   \end{cases}
\]

Or in indicator notation 
$$ u_{m,k} = (x_m - x_k)(2r - d_{m,k}) \mathds{1}_{2r > d_{m,k}}$$

However, it may be that the vector $x_m$ collides with multiple other vectors on any given iteration, so we then have 
$$ u_m = \sum_{k : k \neq m} (x_m - x_k) (2r - d_{m,k}) \mathds{1}_{2r > d_{m,k}}$$

We now update each vector $x_m$ in the configuration, remembering to normalize to ensure that the vector stays on $S^{d - 1}$ 

$$ x_m \xleftarrow{} \frac{x_m + u_m}{|| x_m + u_m ||}$$

After repeating this for each vector in the configuration, we increase the radius by a small amount and repeat on the next iteration. The pseudocode for this algorithm is summarized in \Cref{appendix}, and we have implemented it with efficient vector operations in Pytorch~\citep{pytorch}.


